Explainable Predictive Modeling for Limited Spectral Data

Feature selection of high-dimensional labeled data with limited observations is critical for making powerful predictive modeling accessible, scalable, and interpretable for domain experts. Spectroscopy data, which records the interaction between matter and electromagnetic radiation, particularly holds a lot of information in a single sample. Since acquiring such high-dimensional data is a complex task, it is crucial to exploit the best analytical tools to extract necessary information. In this paper, we investigate the most commonly used feature selection techniques and introduce applying recent explainable AI techniques to interpret the prediction outcomes of high-dimensional and limited spectral data. Interpretation of the prediction outcome is beneficial for the domain experts as it ensures the transparency and faithfulness of the ML models to the domain knowledge. Due to the instrument resolution limitations, pinpointing important regions of the spectroscopy data creates a pathway to optimize the data collection process through the miniaturization of the spectrometer device. Reducing the device size and power and therefore cost is a requirement for the real-world deployment of such a sensor-to-prediction system as a whole. We specifically design three different scenarios to ensure that the evaluation of ML models is robust for the real-time practice of the developed methodologies and to uncover the hidden effect of noise sources on the final outcome.

==> coverletter.tex <==
% \noindent Monday, Jan 10, 2022\\
 \noindent Dr. Roma Tauler\\
{\small
Institute of Environmental Assessment and Water Research, Barcelona, Spain\\
% Email: \\
Editor-in-Chief\\
Chemometrics and Intelligent Laboratory Systems}

% {\bf
% Subject}: {\it Submission of Manuscript ``Explainable Predictive Modeling for Limited Spectral Data'' to Journal of --}

 
\vspace{2mm}
Dear Dr. Tauler,

% \textbf{Authors' Response:}
I am pleased to submit our manuscript, ``Explainable Predictive Modeling for Limited Spectral Data'', for consideration for publication in the Journal of Chemometrics and Intelligent Laboratory Systems.

My co-authors and I believe that the manuscript is suited nicely for the journal’s interdisciplinary approach to share knowledge and report new advances on the Development of statistical, mathematical methods in the Chemometrics discipline.

% on all topics related to information, knowledge engineering and energy systems.
 
Spectroscopy analysis is widely used in various domains to characterize complex chemical processes and reactions. 
Machine learning (ML) is increasingly being used in high-stakes complex applications. There has been increasing interest in applying these ML models for spectral data analysis. While there has been extensive work on developing ML models for predicting spectral data, they elide over the fact that collecting the data is challenging and costly, and blindly applying successful ML models for other domains is not the best action. Despite the high-dimensional nature of these spectra data, the scalability and interpretability of predictive modeling are not discussed or evaluated in the literature.
This paper provides deep insight into the two abovementioned major gaps and conducts a comprehensive study on predictive modeling of spectral data in real-time where the noise is present. We introduce leveraging popular model-agnostic feature selection techniques to predict the Cetane Number of fuels with limited labeled spectral data. 
 


Thank you for considering this manuscript and your work as editor-in-chief of the Journal of Chemometrics and Intelligent Laboratory Systems! Much appreciated!

\textbf{Original Article Statement}
 
a. This manuscript is the authors' original work and has not been published nor has it been submitted simultaneously elsewhere.

b. All authors have checked the manuscript and have agreed to the submission.

{\it\small
\noindent Hadis Anahideh,\\
Research Assistant Professor \\
University of Illinois at Chicago
 }
\newpage
% Enclosures: Manuscript, other required files


==> header.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{pdfpages}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{caption}
\usepackage{rotating}
\usepackage{graphicx}
\usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{caption}
\usepackage{amsmath}

\usepackage{wrapfig}

\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage[table,xcdraw]{xcolor}
\usepackage{mathtools}
\usepackage{lineno}
\usepackage{color}
\usepackage{comment}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm}

% \usepackage[nocompress]{cite}
% \usepackage[numbers]{natbib}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\usepackage{flushend}
%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmaxA}{arg\,max}
\DeclareMathOperator*{\argminA}{arg\,min}
%\newcommand*{\argminl}{\argmin\limits}
%\newcommand*{\argmaxl}{\argmax\limits}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{balance}
\usepackage{enumitem}

\usepackage{capt-of}

\newcommand{\eat}[1]{}
% \newcommand{\techrep}[1]{\textcolor{blue}{#1}}
% \newcommand{\submit}[1]{\textcolor{red}{#1}}
\newcommand{\techrep}[1]{#1}
\newcommand{\submit}[1]{}
\newcommand{\hindent}[1][1]{\hspace{#1\algorithmicindent}}
\newtheorem{theorem}{Theorem} 
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}{Observation}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{problem}{Problem}
\usepackage{array}
\usepackage{xspace}
\usepackage{makecell}
\usepackage{booktabs}

% \newcommand{\getnext}{{\sc get-next}\xspace}
\newcommand{\stitle}[1]{\noindent{\bf #1}}
\newcommand{\overbar}[1]{\mkern1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}


\newcommand\attrib[1]{{\tt \small #1}\xspace}

\graphicspath{ {./figs/} }


==> references.tex <==
% \newpage
% \section{References}

% [1] W.S. McCulloch, W.H. Pitts, A logical calculus of the ideas imminent in nervous activity, Bull. Math. Biophys. 5 (1943) 115–133.

% [2] F. Rosenblatt, The perceptron: a probabilistic model for information storage and organization in the brain, Psychol. Rev. 65 (6) (1958) 386–408.

% [3] Rumelhart, David E.; Hinton, Geoffrey E.; Williams, Ronald J. (1986a). "Learning representations by back-propagating errors". Nature. 323 (6088): 533-536. Bibcode:1986 Nature. 

% [4] Howard, A., Sandler, M., Chu, G., Chen, L.C., Chen, B., Tan, M., Wang, W., Zhu, Y., Pang, R., Vasudevan, V., Le, Q.V., Adam, H., 2019. Searching for MobileNetV3 arXiv:1905.02244.

% [5] Krizhevsky, A., Sutskever, I., Geoffrey E., H., 2012. ImageNet Classification with Deep Convolutional Neural Networks. Advances in Neural Information Processing Systems 25 (NIPS2012) , 1–9

% [6] David Silver, Aja Huang, Chris J. Maddison, Arthur Guez, Laurent Sifre, George van den Driessche, Julian Schrittwieser, Ioannis Antonoglou, Veda Panneershelvam, Marc Lanctot, Sander Dieleman, Dominik Grewe, John Nham, Nal Kalchbrenner, Ilya Sutskever, Timothy Lillicrap, Madeleine Leach, Koray Kavukcuoglu, Thore Graepel \& Demis Hassabis. (2016). Mastering the game of Go with deep neural networks and tree search. Nature. 529. 484-489. 10.1038/nature16961. 

% [7] Mastering Chess and Shogi by Self-Play with a General Reinforcement Learning Algorithm

% [8] Andrew W. Senior, Richard Evans, John Jumper, James Kirkpatrick, Laurent Sifre, Tim Green, Chongli Qin, Augustin Zidek, Alexander W. R. Nelson, Alex Bridgland,
% Hugo Penedones, Stig Petersen, Karen Simonyan, Steve Crossan, Pushmeet Kohli, David T. Jones, David Silver, Koray Kavukcuoglu \& Demis Hassabis.

% [9] Ge Wang. "Humans in the Loop: The Design of Interactive AI Systems". https://hai.stanford.edu/news/humans-loop-design-interactive-ai-systems

% [10] Human-in-the-loop Artificial Intelligence
% Fabio Massimo Zanzotto

% [11] André Meyer-Vitali, Roos Bakker, Michael van Bekkum, Maaike de Boer, Gertjan Burghouts, Jurriaan van Diggelen, Judith Dijk, Corrado Grappiolo, Joachim de Greeff, Albert Huizing, Stephan Raaijmakers. Hybrid AI White Paper

% [12] R.M. Balabin, R.Z. Safieva, Journal of Near Infrared Spectroscopy 343 (2007) 15–20. Capabilities of near Infrared Spectroscopy for the Determination of Petroleum Macromolecule Content in Aromatic Solutions.

% [13] Solomon O. Giwa, Sunday O. Adekomaya, Kayode O. Adama, Moruf O. Mukaila. Energy 2015, 9(4): 433–445. Prediction of selected biodiesel fuel properties using artificial neural network.

% [14] Juan Francisco Garcia-Martin, Francisco Javier Ales-Alvarez, Maria del Carmen Lopez-Barrera, Irene Martin-Dominguez, Paloma Alvarez-Mateos. Cetane number prediction of waste cooking oil-derived biodiesel prior to transesterification reaction using near infrared spectroscopy. Fuel 240 (2019) 10–15

% [15] M. Blanco, J. Coello, H. Iturriaga, S. Maspoch and C. de la Pezuela. Near-infrared spectroscopy in the pharmaceutical industr.

% [16] W. Plugge, C. van der Vliest. The use of near infrared spectroscopy in the quality control laboratory of the pharmaceutical industry. Journal of Pharmaceutical and Biomedical Analysis, Volume 10, Issues 10–12, 1992, Pages 797-803, ISSN 0731-7085.

% [17] Y. Roggo, P. Chalus, L. Maurer, C. Lema-Martinez, A. Edmond, N. Jent, Journal of Pharmaceutical and Biomedical Analysis 44 (2007) 683–700.

% [18] Ernest Teye, Xing-yi Huang, Newlove Afoakwa. Review on the Potential Use of Near Infrared Spectroscopy (NIRS) for the Measurement of Chemical Residues in Food. 

% [19] F.R. van de Voort. Fourier transform infrared spectroscopy applied to food analysis. Food Research International. Volume 25, Issue 5, 1992. Pages 397-403, ISSN 0963-9969.

% [20] Hans Buning-Pfaue. Analysis of water in food by near infrared spectroscopy. Food Chemistry, Volume 82, Issue 1, 2003, Pages 107-115, ISSN 0308-8146.

% [21] Iranian Journal of Pharmaceutical Research (2020), 19 (2): 34-44. Novel Application of Near-infrared Spectroscopy and Chemometrics Approach for Detection of Lime Juice Adulteration.

% [22] Stefano Di Frischia, Paolo Giammatteo, Federico Angelini et al. Enhanced Data Augmentation using GANs for Raman Spectra Classification.

% [23] Zefang Shen \& R. A. Viscarra Rossel. Automated spectroscopic
% modelling with optimised convolutional neural networks. Nature: Scientific Reports. (2021) 11:208.

% %Used PLS, PCA for correlating with fuel sample clustering. trained classifier. 45 samples, 6 octane classes bins (2-4 ON deviation) 
% [24] K. Brudzewski, A. Kesik, K. Kolodziejczyk, U. Zborowska, J. Ulaczyk. Gasoline quality prediction using gas chromatography and FTIR spectroscopy: An artificial intelligence approach. Fuel 85 (2006) 553–558.


% %Analysis of various FS methods, goal: to discard noisy/unnecessary regions, improve prediction performance, scalability, computational efficiency. 612 samples. Methods used: PLS, MLR, SPA, UVE, GA etc. Ultimately showed that PLS is supreme.
% [26] Roman M. Balabin, Sergey V. Smirnov. Variable selection in near-infrared spectroscopy: Benchmarking of feature selection methods on biodiesel data. Analytica Chimica Acta 692 (2011) 63–72.

% [27] Zou Xiaobo, Zhao Jiewen, Malcolm J.W. Povey, Mel Holmes, Mao Hanpin. Variables selection methods in near-infrared spectroscopy. Analytica Chimica Acta 667 (2010) 14–32.

% %Used PCA for reducing features in ANN input. From 401 to 23 wavelengths (5\% of full features). 236 samples. Data was scaled.
% [28] Zvi Boger. Selection of quasi-optimal inputs in chemometrics modeling by artificial neural network analysis. Analytica Chimica Acta 490 (2003) 31–40.

% %Use PLS for FS for efficiency.
% [29] Jeffrey A. Cramer, Kirsten E. Kramer, Kevin J. Johnson, Robert E. Morris, Susan L. Rose-Pehrsson. Automated wavelength selection for spectroscopic fuel models by symmetrically contracting repeated unmoving window partial least squares. Chemometrics and Intelligent Laboratory Systems 92 (2008) 13–21.

% %Gas IR feature selection, 9 features used, such as: chemical functional groups, BI, MW, whose values correlate to PCA/PLS projected latent vectors. 
% [30] Emad Al Ibrahim and Aamir Farooq. Octane Prediction from Infrared Spectroscopic Data. Energy Fuels 2020, 34, 817-826. 

% %These works do CN/ON prediction using PLSR, NN etc. No FS.

% %Using Gas chromatogramy-mass spectrometer:
% [31] Hong Yang , Zbigniew Ring , Yevgenia Briker, Norma McLean, Wally Friesen and Craig Fairbridge. Neural network prediction of cetane number and density of diesel fuel from its chemical composition determined by LC and GC-MS. Fuel 81 (2002) 65-74

% %Using FTIR chemical composition
% [32] C.I. Rocabruno-Valdes, L.F. Ramirez-Verduzco, J.A. Hernandez. Artificial neural network models to predict density, dynamic viscosity, and cetane number of biodiesel. Fuel 147 (2015) 9–17.  

% %Using QSPR analysis:
% [33] Travis Kessler, Eric R. Sacia, Alexis T. Bell, J. Hunter Mack. Artificial neural network based predictions of cetane number for furanic biofuel additives. Fuel 206 (2017) 171–179. 

% %Using Fatty Acid Methyl Esters (FAME) composition
% [34] Ramin Piloto-Rodriguez, Yisel Sanchez-Borroto, Magin Lapuerta, Leonardo Goyos-Perez, Sebastian Verhelst. Prediction of the cetane number of biodiesel using artificial neural networks and multiple linear regression. Energy Conversion and Management 65 (2013) 255–261.

% %Using FTIR spectra and PLS
% [35] Issam Barra, Mourad Kharbach, El Mostafa Qannari, Mohamed Hanafi, Yahia Cherrah, Abdelaziz Bouklouze. Predicting cetane number in diesel fuels using FTIR spectroscopy and PLS regression. Vibrational Spectroscopy 111 (2020) 103157. 

% [36] Xiong Li, YanDe Liu, Xiaogang Jiang, Aiguo Ouyang, Xudong Sun, Guantian Wang. Determination and quantification of kerosene in gasoline by mid-infrared and Raman spectroscopy. Journal of Molecular Structure 1210 (2020) 127760. 


 
% %These are old works on variable selection for spectra using PCA-PLS to make simples models
% [37] D. Jouan-Rimbaud, B. Walczak, D.-L. Massart, I.R. Last, K.A. Prebble, Analytica Chimica Acta 304 (1995) 285–295.

% [38] S.D. Frans, J.M. Harris, Analytical Chemistry 57 (1985) 2680–2684.

% [39] C.H. Spiegelman, M.J. McShane, M.J. Goetz, M. Motamedi, Q.L. Yue, G.L. Cote, Analytical Chemistry 70 (1998) 35–44.

% [40] J.H. Kalivas, N. Roberts, J.M. Sutter, Analytical Chemistry 61 (1989) 2024–2030.

% [41] J.A. Panford, J.M. deMan, Journal of the American Oil Chemists’ Society 67 (1990) 473–482.

% [42] C.W. Brown, P.F. Lynch, R.J. Obremski, D.S. Lavery, Analytical Chemistry 54 (1982) 1472–1479.


% [43] Tan Zhea Ron, Rajasvaran Logeswaran. Interpreting a Neral Network for Stock Data using LIME. Journal of Critical Reviews. Vol 7, Issue 3, 2020. 

% [44] Ihsan Ullah, Andre Rios, Vaibhav Gala and Susan Mckeever. Explaining Deep Learning Models for Structured Data using Layer-Wise Relevance Propagation.

% [45] Pushpa Pandey, Akshay Rai, Mira Mitra. Explainable 1-D convolutional neural network for damage detection using Lamb wave. Mechanical Systems and Signal Processing 164 (2022) 108220. 

% [46] Rohit Saluja, Avleen Malhi, Samanta Knapic, Kary Framling, Cicek Cavdar. Towards a Rigorous Evaluation of Explainability for Multivariate Time Series. 

% [47] Thrun, M.C., Ultsch,A., Breuer, L. Explainable AI Framework for Multivariate Hydrochemical Time Series. Mach. Learn. Knowl. Extr. 2021, 3, 170–204.

% [48] Singh, H., Roy, A., Setia, R.K. et al. Estimation of nitrogen content in wheat from proximal hyperspectral data using machine learning and explainable artificial intelligence (XAI) approach. Model. Earth Syst. Environ. (2021).

% [49] Hirohisa Taniguchi, Tomohiro Takata, Mineki Takechi, Asuka Furukawa, Jin Iwasawa, Akio Kawamura, Tadahiro Taniguchi and Yuichi Tamura. Explainable Artificial Intelligence Model for Diagnosis of Atrial Fibrillation Using Holter Electrocardiogram Waveforms.

% [50] Marco Tulio Ribeiro, Sameer Singh and Carlos Guestrin. "Why Should I Trust You?" Explaining the Predictions of Any Classifier. 

% [54] George Socrates: Infrared and Raman Characteristic Group Frequencies, Third Edition, 2001.

    % [55] A Unified Approach to Interpreting Model Predictions Scott M Lundberg, Su-In Lee

% [56] Predicting Fuel Ignition Quality Using 1H NMR Spectroscopy and Multiple Linear Regression, Abdul Gani Abdul Jameel, Nimal Naser, AbdulHamid Emwas, Stephen Dooley, and S. Mani Sarathy, Energy Fuels 2016, 30, 9819 9835

% [57] A minimalist functional group (MFG) approach for surrogate fuel formulation, Abdul Gani Abdul Jameel a, Nimal Naser a, Gani Issayev a, Jamal Touitou b, Manik Kumer Ghosh b , Abdul-Hamid Emwas c , Aamir Farooq a , Stephen Dooley b , S. Mani Sarathy, Combustion and Flame 192 (2018) 250–271

% [58] A Novel Group Contribution Method for the Prediction of the Derived Cetane Number of Oxygenated Hydrocarbons, Manuel Dahmen and Wolfgang Marquardt, DOI: 10.1021/acs.energyfuels.5b01032 Energy Fuels 2015, 29, 5781 5801

% [59] Combined shifted-excitation Raman difference spectroscopy and support vector regression for monitoring the algal production of complex polysaccharides. Kristina Noack, Bjorn Eskofier, Johannes Kiefer, Christina Dilk, Georg Bilow, Matthias Schirmer, Rainer Buchholz and Alfred Leipertz.

% [60] Determination of diesel quality parameters using support vector regression and near infrared spectroscopy for an in-line blending optimizer system. Julio Cesar L. Alves, Claudete B. Henriques, Ronei J. Poppi

%[61] Support vector machine regression (SVR/LS-SVM)--an alternative to neural networks (ANN) for analytical chemistry? Comparison of nonlinear methods on near infrared (NIR) spectroscopy data. https://eurekamag.com/research/056/016/056016297.php



==> table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|c|r|ccc|ccc|cccr|}
    \toprule
    \multicolumn{1}{|l|}{\multirow{2}[2]{*}{\textbf{Number of samples}}} & \multicolumn{3}{c|}{\multirow{2}[2]{*}{\textbf{145}}} & \multicolumn{3}{c|}{\multirow{2}[2]{*}{\textbf{245}}} & \multicolumn{3}{c|}{\multirow{2}[2]{*}{\textbf{165}}} &       &  \\
          & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} &       &  \\
    \midrule
    \multirow{2}[4]{*}{\textbf{FS method}} & \multicolumn{3}{c|}{\textbf{Control}} & \multicolumn{3}{c|}{\textbf{Mixed}} & \multicolumn{3}{c|}{\textbf{Real-time}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{11}[22]{*}{\begin{sideways}\textbf{BO-Tuned NN}\end{sideways}}} \\
\cmidrule{2-11}          & \multicolumn{1}{c|}{Train MSE ($\mu$,$\sigma$)} & \multicolumn{1}{c|}{\textbf{Test MSE ($\mu$,$\sigma$)}} & \multicolumn{1}{c|}{Time (s)} & Train MSE ($\mu$,$\sigma$) & \multicolumn{1}{c|}{\textbf{Test MSE ($\mu$,$\sigma$)}} & \multicolumn{1}{c|}{Time MSE (s)} & Train MSE ($\mu$,$\sigma$) & \multicolumn{1}{c|}{\textbf{Test MSE ($\mu$,$\sigma$)}} & \multicolumn{1}{c|}{Time (s)} & \multicolumn{1}{c|}{\# parameters} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Full Model} & \multicolumn{1}{c|}{(0.006, 0.004)} & \multicolumn{1}{c|}{(0.04, 0.04)} & \multicolumn{1}{c|}{2338} & (0.02, 0.05) & \multicolumn{1}{c|}{(0.07, 0.13)} & \multicolumn{1}{c|}{2404} & (0.01, 0.01) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(32.3, 6.7)}} & \multicolumn{1}{c|}{2533} & \multicolumn{1}{c|}{11.8 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert } & \multicolumn{1}{c|}{(0.02, 0.006)} & \multicolumn{1}{c|}{(0.04, 0.02)} & \multicolumn{1}{c|}{3506} & (0.02, 0.03) & \multicolumn{1}{c|}{(0.03, 0.15)} & \multicolumn{1}{c|}{4170} & (0.03, 0.02) & \multicolumn{1}{c|}{(64, 19)} & \multicolumn{1}{c|}{2922} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{(0.05, 0.02)} & \multicolumn{1}{c|}{(0.07, 0.03)} & \multicolumn{1}{c|}{3607} & (0.08, 0.02 & \multicolumn{1}{c|}{(0.17, 0.06)} & \multicolumn{1}{c|}{4230} & (0.04, 0.02) & \multicolumn{1}{c|}{(48, 20)} & \multicolumn{1}{c|}{2439} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{(0.29, 0.18)} & \multicolumn{1}{c|}{(0.5, 0.58)} & \multicolumn{1}{c|}{3896} & (2.07, 0.85) & \multicolumn{1}{c|}{(1.6, 1)} & \multicolumn{1}{c|}{4832} & (1.66, 0.7) & \multicolumn{1}{c|}{(92, 17.2)} & \multicolumn{1}{c|}{2835} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{(0.05, 0.01)} & \multicolumn{1}{c|}{(0.08, 0.03)} & \multicolumn{1}{c|}{3421} & (0.04, 0.02) & \multicolumn{1}{c|}{(0.06, 0.02)} & \multicolumn{1}{c|}{4260} & (0.09, 0.08) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(39.5, 12.8)}} & \multicolumn{1}{c|}{2421} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{(0.05, 0.03)} & \multicolumn{1}{c|}{(0.07, 0.03)} & \multicolumn{1}{c|}{3327} & (0.05, 0.01) & \multicolumn{1}{c|}{(0.07, 0.03)} & \multicolumn{1}{c|}{4122} & (0.06, 0.07) & \multicolumn{1}{c|}{(58.5, 20.6)} & \multicolumn{1}{c|}{2855} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{(0.04, 0.02)} & \multicolumn{1}{c|}{(0.05, 0.02)} & \multicolumn{1}{c|}{3266} & (0.02, 0.01) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.02, 0.01)}} & \multicolumn{1}{c|}{4620} & (0.04, 0.025) & \multicolumn{1}{c|}{(46, 32)} & \multicolumn{1}{c|}{2806} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{(0.04, 0.01)} & \multicolumn{1}{c|}{(0.06, 0.03)} & \multicolumn{1}{c|}{3285} & (0.04, 0.02) & \multicolumn{1}{c|}{(0.06, 0.02)} & \multicolumn{1}{c|}{4410} & (0.03, 0.027) & \multicolumn{1}{c|}{(50, 12)} & \multicolumn{1}{c|}{2460} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{(0.03, 0.01)} & \multicolumn{1}{c|}{(0.05, 0.03)} & \multicolumn{1}{c|}{3217} & (0.05, 0.02) & \multicolumn{1}{c|}{(0.09, 0.03)} & \multicolumn{1}{c|}{4350} & (0.06, 0.035) & \multicolumn{1}{c|}{(52, 14)} & \multicolumn{1}{c|}{2444} & \multicolumn{1}{c|}{13.1 mil} &  \\
    \midrule
    \textbf{Avg. runtime} & \multicolumn{1}{r}{} &       & \textbf{111} &       &       & \textbf{139} &       &       & \textbf{88} &       &  \\
    \midrule
    \multicolumn{1}{|l|}{Full Model} & \multicolumn{1}{c|}{(0.006, 0.004)} & \multicolumn{1}{c|}{(0.04, 0.04)} & \multicolumn{1}{c|}{2404} & (0.024, 0.045) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.07, 0.127)}} & \multicolumn{1}{c|}{2617} & (0.01, 0.01) & \multicolumn{1}{c|}{(32.3, 6.7)} & \multicolumn{1}{c|}{2613} & \multicolumn{1}{c|}{11.8 mil} & \multicolumn{1}{c|}{\multirow{9}[18]{*}{\begin{sideways}\textbf{Ridgid-Tuned NN}\end{sideways}}} \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert Features} & \multicolumn{1}{c|}{(0.05, 0.03)} & \multicolumn{1}{c|}{(0.25, 0.2)} & \multicolumn{1}{c|}{344} & (0.19, 0.35) & \multicolumn{1}{c|}{(0.26, 0.5)} & \multicolumn{1}{c|}{375} & (5, 1) & \multicolumn{1}{c|}{(63.7, 3)} & \multicolumn{1}{c|}{351} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{(1.3, 0.3)} & \multicolumn{1}{c|}{(4.9, 2.5)} & \multicolumn{1}{c|}{380} & (0.5, 0.83) & \multicolumn{1}{c|}{(0.67, 1.1)} & \multicolumn{1}{c|}{391} & (0.21, 0.5) & \multicolumn{1}{c|}{(42.6, 11)} & \multicolumn{1}{c|}{381} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{(22, 15)} & \multicolumn{1}{c|}{(19, 20)} & \multicolumn{1}{c|}{391} & (12.3, 1.9) & \multicolumn{1}{c|}{(13.9, 4.6)} & \multicolumn{1}{c|}{462} & (11.7, 0.68) & \multicolumn{1}{c|}{(73.8, 7.2)} & \multicolumn{1}{c|}{366} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{(0.86, 1.15)} & \multicolumn{1}{c|}{(1.62, 1.9)} & \multicolumn{1}{c|}{377} & (4.6, 0.8) & \multicolumn{1}{c|}{(5.7, 1.9)} & \multicolumn{1}{c|}{358} & (0.73, 1.32) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(16, 1)}} & \multicolumn{1}{c|}{456} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{(0.73, 0.96)} & \multicolumn{1}{c|}{(2.7, 3.8)} & \multicolumn{1}{c|}{361} & (0.6, 0.96) & \multicolumn{1}{c|}{(1.03, 1.95)} & \multicolumn{1}{c|}{377} & (3, 0.34) & \multicolumn{1}{c|}{(31.7, 2)} & \multicolumn{1}{c|}{396} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{(0.001, 0.0015)} & \multicolumn{1}{c|}{(0.06, 0.13)} & \multicolumn{1}{c|}{384} & (0.67, 0.87) & \multicolumn{1}{c|}{(0.82, 0.996)} & \multicolumn{1}{c|}{470} & (3, 0.4) & \multicolumn{1}{c|}{(38.6, 0.9)} & \multicolumn{1}{c|}{357} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{(0.001, 0.008)} & \multicolumn{1}{c|}{(0.02, 0.029)} & \multicolumn{1}{c|}{362} & (0.83, 1.19) & \multicolumn{1}{c|}{(0.83, 1.07)} & \multicolumn{1}{c|}{383} & (0.35, 0.63) & \multicolumn{1}{c|}{(38, 2.1)} & \multicolumn{1}{c|}{369} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{(0.048, 0.07)} & \multicolumn{1}{c|}{(0.225, 0.18)} & \multicolumn{1}{c|}{366} & (0.42, 0.72) & \multicolumn{1}{c|}{(0.5, 0.67)} & \multicolumn{1}{c|}{376} & (0.13, 0.43) & \multicolumn{1}{c|}{(38, 2.3)} & \multicolumn{1}{c|}{333} & \multicolumn{1}{c|}{0.5 mil} &  \\
    \midrule
    \textbf{Avg. runtime} &       &       & \textbf{19.89} &       &       & \textbf{21.51} &       &       & \textbf{20.82} &       &  \\
    \midrule
    \multicolumn{1}{|l|}{Full Model} & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.02, 0.008)} & \multicolumn{1}{c|}{0.58} & (0.007, 0.0002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.05, 0.019)}} & \multicolumn{1}{c|}{11.4} & (0.006, 0.002) & \multicolumn{1}{c|}{(33.67, 5.44)} & \multicolumn{1}{c|}{0.63} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{9}[18]{*}{\begin{sideways}\textbf{Optimized SVR}\end{sideways}}} \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert Features} & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.02, 0.009)} & \multicolumn{1}{c|}{1.2} & (0.01, 0.007) & \multicolumn{1}{c|}{(0.05, 0.02)} & \multicolumn{1}{c|}{35.97} & (0.006, 0.002) & \multicolumn{1}{c|}{(33.95, 6.4)} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{(0.007, 0.002)} & \multicolumn{1}{c|}{(0.04, 0.015)} & \multicolumn{1}{c|}{2.75} & (0.026, 0.04) & \multicolumn{1}{c|}{(0.1, 0.08)} & \multicolumn{1}{c|}{42.25} & (0.007, 0.002) & \multicolumn{1}{c|}{(34, 5.5)} & \multicolumn{1}{c|}{2.65} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{(0.016, 0.007)} & \multicolumn{1}{c|}{(0.32, 0.115)} & \multicolumn{1}{c|}{30.8} & (1.3, 1.5) & \multicolumn{1}{c|}{(2.46, 2.3)} & \multicolumn{1}{c|}{61.12} & (0.016, 0.007) & \multicolumn{1}{c|}{(42.5, 9.2)} & \multicolumn{1}{c|}{30.27} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{(0.008, 0.002)} & \multicolumn{1}{c|}{(0.06, 0.03)} & \multicolumn{1}{c|}{5.2} & (0.8, 0.74) & \multicolumn{1}{c|}{(0.36, 0.22)} & \multicolumn{1}{c|}{56.78} & (0.008, 0.002) & \multicolumn{1}{c|}{(41.2, 2.1)} & \multicolumn{1}{c|}{5.35} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{(0.006, 0.003)} & \multicolumn{1}{c|}{(0.03, 0.013)} & \multicolumn{1}{c|}{1.3} & (0.07, 0.07) & \multicolumn{1}{c|}{(0.13, 0.08)} & \multicolumn{1}{c|}{41.97} & (0.007, 0.003) & \multicolumn{1}{c|}{(37.9, 9.1)} & \multicolumn{1}{c|}{1.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.03, 0.01)} & \multicolumn{1}{c|}{1.8} & (0.11, 0.3) & \multicolumn{1}{c|}{(0.46, 1.83)} & \multicolumn{1}{c|}{39.84} & (0.006, 0.002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(32.85, 4.7)}} & \multicolumn{1}{c|}{1.83} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.03, 0.013)} & \multicolumn{1}{c|}{1.7} & (0.14, 0.58) & \multicolumn{1}{c|}{(0.44, 1.67)} & \multicolumn{1}{c|}{38.93} & (0.007, 0.003) & \multicolumn{1}{c|}{(36, 6.3)} & \multicolumn{1}{c|}{1.63} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.02, 0.008)} & \multicolumn{1}{c|}{1} & (0.027, 0.06) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.08, 0.05)}} & \multicolumn{1}{c|}{37.63} & (0.006, 0.002) & \multicolumn{1}{c|}{(36, 3.74)} & \multicolumn{1}{c|}{1.06} & \multicolumn{1}{c|}{} &  \\
    \midrule
    \textbf{Avg. runtime} &       &       & \textbf{0.17} &       &       & \textbf{1.4} &       &       & \textbf{0.2} &       &  \\
    \midrule
    \multicolumn{1}{|l|}{Full Model} & \multicolumn{1}{c|}{(0.07, 0.001)} & \multicolumn{1}{c|}{(0.08, 0.02)} & \multicolumn{1}{c|}{0.41} & (0.007, 0.0002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.11, 0.03)}} & \multicolumn{1}{c|}{5.18} & (0.006, 0.002) & \multicolumn{1}{c|}{(14.8, 1.1)} & \multicolumn{1}{c|}{0.45} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{9}[18]{*}{\begin{sideways}\textbf{Tuned SVR}\end{sideways}}} \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert Features} & \multicolumn{1}{c|}{(0.06, 0.001)} & \multicolumn{1}{c|}{(0.08, 0.02)} & \multicolumn{1}{c|}{0.36} & (0.06, 0.001) & \multicolumn{1}{c|}{(0.11, 0.04)} & \multicolumn{1}{c|}{17.2} & (0.006, 0.002) & \multicolumn{1}{c|}{(14, 2.1)} & \multicolumn{1}{c|}{0.36} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{(0.07, 0.003)} & \multicolumn{1}{c|}{(0.11, 0.03)} & \multicolumn{1}{c|}{0.97} & (0.06, 0.002) & \multicolumn{1}{c|}{(0.1, 0.08)} & \multicolumn{1}{c|}{24.1} & (0.007, 0.002) & \multicolumn{1}{c|}{(15.2, 1.2)} & \multicolumn{1}{c|}{0.98} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{(0.07, 0.003)} & \multicolumn{1}{c|}{(0.13, 0.04)} & \multicolumn{1}{c|}{5.1} & (1, 0.79) & \multicolumn{1}{c|}{(1.5, 0.9)} & \multicolumn{1}{c|}{39.2} & (0.016, 0.007) & \multicolumn{1}{c|}{(16.2, 1.4)} & \multicolumn{1}{c|}{5} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{(0.06, 0.002)} & \multicolumn{1}{c|}{(0.08, 0.03)} & \multicolumn{1}{c|}{0.49} & (0.06, 0.001) & \multicolumn{1}{c|}{(0.09, 0.02)} & \multicolumn{1}{c|}{5.5} & (0.008, 0.002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(4.6, 0.2)}} & \multicolumn{1}{c|}{0.5} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{(0.06, 0.002)} & \multicolumn{1}{c|}{(0.08, 0.02)} & \multicolumn{1}{c|}{0.37} & (0.06, 0.001) & \multicolumn{1}{c|}{(0.1, 0.03)} & \multicolumn{1}{c|}{7.9} & (0.007, 0.003) & \multicolumn{1}{c|}{(11.8, 0.7)} & \multicolumn{1}{c|}{0.37} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{(0.07, 0.003)} & \multicolumn{1}{c|}{(0.1, 0.03)} & \multicolumn{1}{c|}{0.7} & (0.06, 0.002) & \multicolumn{1}{c|}{(0.14, 0.05)} & \multicolumn{1}{c|}{22.3} & (0.006, 0.002) & \multicolumn{1}{c|}{(12.5, 0.7)} & \multicolumn{1}{c|}{0.73} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{(0.06, 0.002)} & \multicolumn{1}{c|}{(0.1, 0.02)} & \multicolumn{1}{c|}{0.68} & (0.06, 0.002) & \multicolumn{1}{c|}{(0.12, 0.04)} & \multicolumn{1}{c|}{16.1} & (0.007, 0.003) & \multicolumn{1}{c|}{(11.8, 1.1)} & \multicolumn{1}{c|}{0.7} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{(0.06, 0.002)} & \multicolumn{1}{c|}{(0.1, 0.02)} & \multicolumn{1}{c|}{0.56} & (0.06, 0.002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.12, 0.03)}} & \multicolumn{1}{c|}{14.7} & (0.006, 0.002) & \multicolumn{1}{c|}{(13.9, 0.9)} & \multicolumn{1}{c|}{0.55} & \multicolumn{1}{c|}{} &  \\
    \midrule
    \textbf{Avg. runtime} &       &       & \textbf{0.04} &       &       & \textbf{0.6} &       &       & \textbf{0.0} &       &  \\
    \midrule
    \multicolumn{1}{|l|}{Full Model} & \multicolumn{1}{c|}{e\^-27} & \multicolumn{1}{c|}{(0.02, 0.01)} & \multicolumn{1}{c|}{0.74} & e\^-26 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.18, 0.06)}} & \multicolumn{1}{c|}{1.28} & e\^-27 & \multicolumn{1}{c|}{(88.8, 6.5)} & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{9}[18]{*}{\begin{sideways}\textbf{LR}\end{sideways}}} \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert} & \multicolumn{1}{c|}{e\^-26} & \multicolumn{1}{c|}{(0.64, 0.65)} & \multicolumn{1}{c|}{0.33} & (0.06, 0.005) & \multicolumn{1}{c|}{(0.35, 0.1)} & \multicolumn{1}{c|}{0.39} & e\^-27 & \multicolumn{1}{c|}{(451, 590)} & \multicolumn{1}{c|}{0.43} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{e\^-26} & \multicolumn{1}{c|}{(3.6, 3.6)} & \multicolumn{1}{c|}{0.34} & (0.16, 0.017) & \multicolumn{1}{c|}{(1.13, 0.36)} & \multicolumn{1}{c|}{0.39} & e\^-25 & \multicolumn{1}{c|}{(1069, 1741)} & \multicolumn{1}{c|}{0.34} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{e\^-25} & \multicolumn{1}{c|}{(19, 17)} & \multicolumn{1}{c|}{0.33} & (0.39, 0.03) & \multicolumn{1}{c|}{(2.5, 0.7)} & \multicolumn{1}{c|}{0.39} & e\^-25 & \multicolumn{1}{c|}{(243, 163)} & \multicolumn{1}{c|}{0.34} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{e\^-26} & \multicolumn{1}{c|}{(5.2, 4.6)} & \multicolumn{1}{c|}{0.33} & (0.19, 0.02) & \multicolumn{1}{c|}{(1.3, 0.4)} & \multicolumn{1}{c|}{0.4} & e\^-26 & \multicolumn{1}{c|}{(233, 427)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{e\^-26} & \multicolumn{1}{c|}{(0.38, 0.65)} & \multicolumn{1}{c|}{0.35} & (0.09, 0.01) & \multicolumn{1}{c|}{(0.67, 0.21)} & \multicolumn{1}{c|}{0.39} & e\^-26 & \multicolumn{1}{c|}{(265, 317)} & \multicolumn{1}{c|}{0.34} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP w/h SVR} & \multicolumn{1}{c|}{e\^-26} & \multicolumn{1}{c|}{(1, 0.7)} & \multicolumn{1}{c|}{0.34} & (0.09, 0.01) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.66, 0.24)}} & \multicolumn{1}{c|}{0.41} & e\^-26 & \multicolumn{1}{c|}{(464, 479)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS w/h SVR} & \multicolumn{1}{c|}{e\^-25} & \multicolumn{1}{c|}{(2.55, 2.3)} & \multicolumn{1}{c|}{0.33} & (0.12, 0.01) & \multicolumn{1}{c|}{(0.72, 0.2)} & \multicolumn{1}{c|}{0.39} & e\^-25 & \multicolumn{1}{c|}{(2280, 3976)} & \multicolumn{1}{c|}{0.34} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME w/h SVR} & \multicolumn{1}{c|}{e\^-26} & \multicolumn{1}{c|}{(2.27, 1.3)} & \multicolumn{1}{c|}{0.32} & (0.1, 0.01) & \multicolumn{1}{c|}{(0.7, 0.2)} & \multicolumn{1}{c|}{0.39} & e\^-26 & \multicolumn{1}{c|}{(2853, 5125)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
    \midrule
    \textbf{Avg. runtime} &       &       & \textbf{0.01} &       &       & \textbf{0.02} &       &       & \textbf{0.01} &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> table_old.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
    \begin{tabular}{|rr|ccc|ccc|cccr|}
    \toprule
    \multicolumn{1}{|c|}{\multirow{2}[2]{*}{\textbf{Number of samples}}} & \multicolumn{3}{c|}{\multirow{2}[2]{*}{\textbf{145}}} & \multicolumn{3}{c|}{\multirow{2}[2]{*}{\textbf{245}}} & \multicolumn{3}{c|}{\multirow{2}[2]{*}{\textbf{165}}} &       &  \\
    \multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} &       &  \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{FS method}}} & \multicolumn{3}{c|}{\textbf{Control}} & \multicolumn{3}{c|}{\textbf{Mixed}} & \multicolumn{3}{c|}{\textbf{Real-time}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{11}[22]{*}{\begin{sideways}\textbf{Shallow NN}\end{sideways}}} \\
\cmidrule{2-11}    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{Train ($\mu$,$\sigma$)} & \multicolumn{1}{c|}{\textbf{Test ($\mu$,$\sigma$)}} & \multicolumn{1}{c|}{Time (s)} & Train ($\mu$,$\sigma$) & \multicolumn{1}{c|}{\textbf{Test ($\mu$,$\sigma$)}} & \multicolumn{1}{c|}{Time (s)} & Train ($\mu$,$\sigma$) & \multicolumn{1}{c|}{\textbf{Test ($\mu$,$\sigma$)}} & \multicolumn{1}{c|}{Time (s)} & \multicolumn{1}{c|}{\# parameters} &  \\
\cmidrule{1-11}    \multicolumn{1}{|c|}{Full Model} & \multicolumn{1}{c|}{(0.006, 0.004)} & \multicolumn{1}{c|}{(0.04, 0.04)} & \multicolumn{1}{c|}{2404} & (0.024, 0.045) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.07, 0.127)}} & \multicolumn{1}{c|}{2730} & (0.01, 0.01) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(32.3, 6.7)}} & \multicolumn{1}{c|}{2613} & \multicolumn{1}{c|}{11.8 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert } & \multicolumn{1}{c|}{(0.05, 0.03)} & \multicolumn{1}{c|}{(0.25, 0.2)} & \multicolumn{1}{c|}{344} & (0.19, 0.35) & \multicolumn{1}{c|}{(0.26, 0.5)} & \multicolumn{1}{c|}{375} & (5, 1) & \multicolumn{1}{c|}{(63.7, 3)} & \multicolumn{1}{c|}{351} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{(1.3, 0.3)} & \multicolumn{1}{c|}{(4.9, 2.5)} & \multicolumn{1}{c|}{380} & (0.5, 0.83) & \multicolumn{1}{c|}{(0.67, 1.1)} & \multicolumn{1}{c|}{391} & (0.21, 0.5) & \multicolumn{1}{c|}{(42.6, 11)} & \multicolumn{1}{c|}{381} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{(22, 15)} & \multicolumn{1}{c|}{(19, 20)} & \multicolumn{1}{c|}{391} & (12.3, 1.9) & \multicolumn{1}{c|}{(13.9, 4.6)} & \multicolumn{1}{c|}{388} & (11.7, 0.68) & \multicolumn{1}{c|}{(73.8, 7.2)} & \multicolumn{1}{c|}{366} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{(0.86, 1.15)} & \multicolumn{1}{c|}{(1.62, 1.9)} & \multicolumn{1}{c|}{377} & (4.6, 0.8) & \multicolumn{1}{c|}{(6, 2.5)} & \multicolumn{1}{c|}{349} & (0.73, 1.32) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(16, 1)}} & \multicolumn{1}{c|}{456} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{(0.73, 0.96)} & \multicolumn{1}{c|}{(2.7, 3.8)} & \multicolumn{1}{c|}{361} & (0.6, 0.96) & \multicolumn{1}{c|}{(1.03, 1.95)} & \multicolumn{1}{c|}{353} & (3, 0.34) & \multicolumn{1}{c|}{(31.7, 2)} & \multicolumn{1}{c|}{396} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{(0.001, 0.0015)} & \multicolumn{1}{c|}{(0.06, 0.13)} & \multicolumn{1}{c|}{384} & (0.67, 0.87) & \multicolumn{1}{c|}{(0.82, 0.996)} & \multicolumn{1}{c|}{470} & (3, 0.4) & \multicolumn{1}{c|}{(38.6, 0.9)} & \multicolumn{1}{c|}{357} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{(0.001, 0.008)} & \multicolumn{1}{c|}{(0.02, 0.029)} & \multicolumn{1}{c|}{362} & (0.83, 1.19) & \multicolumn{1}{c|}{(0.83, 1.07)} & \multicolumn{1}{c|}{383} & (0.35, 0.63) & \multicolumn{1}{c|}{(38, 2.1)} & \multicolumn{1}{c|}{369} & \multicolumn{1}{c|}{0.5 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{(0.048, 0.07)} & \multicolumn{1}{c|}{(0.225, 0.18)} & \multicolumn{1}{c|}{366} & (0.42, 0.72) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.5, 0.67)}} & \multicolumn{1}{c|}{376} & (0.13, 0.43) & \multicolumn{1}{c|}{(38, 2.3)} & \multicolumn{1}{c|}{333} & \multicolumn{1}{c|}{0.5 mil} &  \\
    \midrule
          &       & \textbf{Avg. runtime} & \textbf{20} &       & \textbf{Avg. runtime} & \textbf{22} &       & \textbf{Avg. runtime} & \textbf{21} &       &  \\
    \midrule
    \multicolumn{1}{|c|}{Full Model} & \multicolumn{1}{c|}{(0.006, 0.004)} & \multicolumn{1}{c|}{(0.04, 0.04)} & \multicolumn{1}{c|}{2338} & (0.02, 0.05) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.07, 0.13)}} & \multicolumn{1}{c|}{2404} & (0.01, 0.01) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(32.3, 6.7)}} & \multicolumn{1}{c|}{2533} & \multicolumn{1}{c|}{11.8 mil} & \multicolumn{1}{c|}{\multirow{9}[18]{*}{\begin{sideways}\textbf{Deep NN}\end{sideways}}} \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert Features} & \multicolumn{1}{c|}{(0.02, 0.006)} & \multicolumn{1}{c|}{(0.04, 0.02)} & \multicolumn{1}{c|}{3506} & (0.02, 0.03) & \multicolumn{1}{c|}{(0.03, 0.15)} & \multicolumn{1}{c|}{4170} & (0.03, 0.02) & \multicolumn{1}{c|}{(64, 19)} & \multicolumn{1}{c|}{2922} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{(0.05, 0.02)} & \multicolumn{1}{c|}{(0.07, 0.03)} & \multicolumn{1}{c|}{3607} & (0.08, 0.02 & \multicolumn{1}{c|}{(0.17, 0.06)} & \multicolumn{1}{c|}{4230} & (0.04, 0.02) & \multicolumn{1}{c|}{(48, 20)} & \multicolumn{1}{c|}{2439} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{(0.29, 0.18)} & \multicolumn{1}{c|}{(0.5, 0.58)} & \multicolumn{1}{c|}{3896} & (2.07, 0.85) & \multicolumn{1}{c|}{(1.6, 1)} & \multicolumn{1}{c|}{4832} & (1.66, 0.7) & \multicolumn{1}{c|}{(92, 17.2)} & \multicolumn{1}{c|}{2835} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{(0.05, 0.01)} & \multicolumn{1}{c|}{(0.08, 0.03)} & \multicolumn{1}{c|}{3421} & (0.04, 0.02) & \multicolumn{1}{c|}{(0.06, 0.02)} & \multicolumn{1}{c|}{4260} & (0.09, 0.08) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(39.5, 12.8)}} & \multicolumn{1}{c|}{2421} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{(0.05, 0.03)} & \multicolumn{1}{c|}{(0.07, 0.03)} & \multicolumn{1}{c|}{3327} & (0.05, 0.01) & \multicolumn{1}{c|}{(0.07, 0.03)} & \multicolumn{1}{c|}{4122} & (0.06, 0.07) & \multicolumn{1}{c|}{(58.5, 20.6)} & \multicolumn{1}{c|}{2855} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{(0.04, 0.02)} & \multicolumn{1}{c|}{(0.05, 0.02)} & \multicolumn{1}{c|}{3266} & (0.02, 0.01) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.02, 0.01)}} & \multicolumn{1}{c|}{4620} & (0.04, 0.025) & \multicolumn{1}{c|}{(46, 32)} & \multicolumn{1}{c|}{2806} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{(0.04, 0.01)} & \multicolumn{1}{c|}{(0.06, 0.03)} & \multicolumn{1}{c|}{3285} & (0.04, 0.02) & \multicolumn{1}{c|}{(0.06, 0.02)} & \multicolumn{1}{c|}{4410} & (0.03, 0.027) & \multicolumn{1}{c|}{(50, 12)} & \multicolumn{1}{c|}{2460} & \multicolumn{1}{c|}{13.1 mil} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{(0.03, 0.01)} & \multicolumn{1}{c|}{(0.05, 0.03)} & \multicolumn{1}{c|}{3217} & (0.05, 0.02) & \multicolumn{1}{c|}{(0.09, 0.03)} & \multicolumn{1}{c|}{4350} & (0.06, 0.035) & \multicolumn{1}{c|}{(52, 14)} & \multicolumn{1}{c|}{2444} & \multicolumn{1}{c|}{13.1 mil} &  \\
    \midrule
          &       & \textbf{Avg. runtime} & \textbf{110.60} &       & \textbf{Avg. runtime} & \textbf{138.51} &       & \textbf{Avg. runtime} & \textbf{87.83} &       &  \\
    \midrule
    \multicolumn{1}{|c|}{Full Model} & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.02, 0.008)} & \multicolumn{1}{c|}{0.58} & (0.007, 0.0002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.05, 0.019)}} & \multicolumn{1}{c|}{11.4} & (0.006, 0.002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(33.67, 5.44)}} & \multicolumn{1}{c|}{0.63} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{9}[18]{*}{\begin{sideways}\textbf{SVR}\end{sideways}}} \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert Features} & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.02, 0.009)} & \multicolumn{1}{c|}{1.2} & (0.01, 0.007) & \multicolumn{1}{c|}{(0.05, 0.02)} & \multicolumn{1}{c|}{35.97} & (0.006, 0.002) & \multicolumn{1}{c|}{(33.95, 6.4)} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{(0.007, 0.002)} & \multicolumn{1}{c|}{(0.04, 0.015)} & \multicolumn{1}{c|}{2.75} & (0.026, 0.04) & \multicolumn{1}{c|}{(0.1, 0.08)} & \multicolumn{1}{c|}{42.25} & (0.007, 0.002) & \multicolumn{1}{c|}{(34, 5.5)} & \multicolumn{1}{c|}{2.65} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{(0.016, 0.007)} & \multicolumn{1}{c|}{(0.32, 0.115)} & \multicolumn{1}{c|}{30.8} & (1.3, 1.5) & \multicolumn{1}{c|}{(2.46, 2.3)} & \multicolumn{1}{c|}{61.12} & (0.016, 0.007) & \multicolumn{1}{c|}{(42.5, 9.2)} & \multicolumn{1}{c|}{30.27} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{(0.008, 0.002)} & \multicolumn{1}{c|}{(0.06, 0.03)} & \multicolumn{1}{c|}{5.2} & (0.8, 0.74) & \multicolumn{1}{c|}{(1.57, 1.48)} & \multicolumn{1}{c|}{56.78} & (0.008, 0.002) & \multicolumn{1}{c|}{(41.2, 2.1)} & \multicolumn{1}{c|}{5.35} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{(0.006, 0.003)} & \multicolumn{1}{c|}{(0.03, 0.013)} & \multicolumn{1}{c|}{1.3} & (0.07, 0.07) & \multicolumn{1}{c|}{(0.13, 0.08)} & \multicolumn{1}{c|}{41.97} & (0.007, 0.003) & \multicolumn{1}{c|}{(37.9, 9.1)} & \multicolumn{1}{c|}{1.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.03, 0.01)} & \multicolumn{1}{c|}{1.8} & (0.11, 0.3) & \multicolumn{1}{c|}{(0.46, 1.83)} & \multicolumn{1}{c|}{39.84} & (0.006, 0.002) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(32.85, 4.7)}} & \multicolumn{1}{c|}{1.83} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.03, 0.013)} & \multicolumn{1}{c|}{1.7} & (0.14, 0.58) & \multicolumn{1}{c|}{(0.44, 1.67)} & \multicolumn{1}{c|}{38.93} & (0.007, 0.003) & \multicolumn{1}{c|}{(36, 6.3)} & \multicolumn{1}{c|}{1.63} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{(0.006, 0.002)} & \multicolumn{1}{c|}{(0.02, 0.008)} & \multicolumn{1}{c|}{1} & (0.027, 0.06) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.08, 0.05)}} & \multicolumn{1}{c|}{37.63} & (0.006, 0.002) & \multicolumn{1}{c|}{(36, 3.74)} & \multicolumn{1}{c|}{1.06} & \multicolumn{1}{c|}{} &  \\
    \midrule
          &       & \textbf{Avg. runtime} & \textbf{0.17} &       & \textbf{Avg. runtime} & \textbf{1.4} &       & \textbf{Avg. runtime} & \textbf{0.2} &       &  \\
    \midrule
    \multicolumn{1}{|c|}{Full Model} & \multicolumn{1}{c|}{$e^{-27}$} & \multicolumn{1}{c|}{(0.02, 0.01)} & \multicolumn{1}{c|}{0.74} & $e^{-26}$ & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.18, 0.06)}} & \multicolumn{1}{c|}{1.28} & $e^{-27}$ & \multicolumn{1}{c|}{(88.8, 6.5)} & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{9}[18]{*}{\begin{sideways}\textbf{LR}\end{sideways}}} \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Expert Features} & \multicolumn{1}{c|}{$e^{-26}$} & \multicolumn{1}{c|}{(0.64, 0.65)} & \multicolumn{1}{c|}{0.33} & (0.06, 0.005) & \multicolumn{1}{c|}{(0.35, 0.1)} & \multicolumn{1}{c|}{0.39} & $e^{-27}$ & \multicolumn{1}{c|}{(451, 590)} & \multicolumn{1}{c|}{0.43} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PCA} & \multicolumn{1}{c|}{$e^{-26}$} & \multicolumn{1}{c|}{(3.6, 3.6)} & \multicolumn{1}{c|}{0.34} & (0.16, 0.017) & \multicolumn{1}{c|}{(1.13, 0.36)} & \multicolumn{1}{c|}{0.39} & $e^{-27}$ & \multicolumn{1}{c|}{(2498, 3396)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{PLS} & \multicolumn{1}{c|}{e\^-25} & \multicolumn{1}{c|}{(19, 17)} & \multicolumn{1}{c|}{0.33} & (0.39, 0.03) & \multicolumn{1}{c|}{(2.5, 0.7)} & \multicolumn{1}{c|}{0.39} & $e^{-27}$ & \multicolumn{1}{c|}{(2498, 3396)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{RF} & \multicolumn{1}{c|}{$e^{-26}$} & \multicolumn{1}{c|}{(5.2, 4.6)} & \multicolumn{1}{c|}{0.33} & (0.19, 0.02) & \multicolumn{1}{c|}{(1.3, 0.4)} & \multicolumn{1}{c|}{0.4} & $e^{-27}$ & \multicolumn{1}{c|}{(2498, 3396)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{Ridge} & \multicolumn{1}{c|}{$e^{-26}$} & \multicolumn{1}{c|}{(0.38, 0.65)} & \multicolumn{1}{c|}{0.35} & (0.09, 0.01) & \multicolumn{1}{c|}{(0.67, 0.21)} & \multicolumn{1}{c|}{0.39} & $e^{-27}$ & \multicolumn{1}{c|}{(2498, 3396)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{SHAP } & \multicolumn{1}{c|}{$e^{-26}$} & \multicolumn{1}{c|}{(1, 0.7)} & \multicolumn{1}{c|}{0.34} & (0.09, 0.01) & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{(0.66, 0.24)}} & \multicolumn{1}{c|}{0.41} & $e^{-27}$ & \multicolumn{1}{c|}{(2498, 3396)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{GS } & \multicolumn{1}{c|}{e\^-25} & \multicolumn{1}{c|}{(2.55, 2.3)} & \multicolumn{1}{c|}{0.33} & (0.12, 0.01) & \multicolumn{1}{c|}{(0.72, 0.2)} & \multicolumn{1}{c|}{0.39} & $e^{-27}$ & \multicolumn{1}{c|}{(2498, 3396)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
\cmidrule{1-11}    \multicolumn{1}{|l|}{LIME } & \multicolumn{1}{c|}{$e^{-26}$} & \multicolumn{1}{c|}{(2.27, 1.3)} & \multicolumn{1}{c|}{0.32} & (0.1, 0.01) & \multicolumn{1}{c|}{(0.7, 0.2)} & \multicolumn{1}{c|}{0.39} & $e^{-27}$ & \multicolumn{1}{c|}{(2498, 3396)} & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{} &  \\
    \midrule
          &       & \textbf{Avg. runtime} & \textbf{0.01} &       & \textbf{Avg. runtime} & \textbf{0.02} &       & \textbf{Avg. runtime} & \textbf{0.01} &       &  \\
    \bottomrule
    \end{tabular}%
\caption{Performance of NN, SVR and LR predictive models fitted with Full and Reduced sets of features measured using mean training and testing error ($\mu$ MSE) with corresponding mean deviation across 30 random splits of data ($\sigma$)}
\label{tab:finalResults}%
\end{table*}%



